Blockchain meets Biometrics: Concepts, Application to Template Protection, and Trends

Blockchain technologies provide excellent architectures and practical tools for securing and managing the sensitive and private data stored in biometric templates, but at a cost. We discuss opportunities and challenges in the integration of blockchain and biometrics, with emphasis in biometric template storage and protection, a key problem in biometrics still largely unsolved. Key tradeoffs involved in that integration, namely, latency, processing time, economic cost, and biometric performance are experimentally studied through the implementation of a smart contract on the Ethereum blockchain platform, which is publicly available in github for research purposes.

==> Reviewers_response.tex <==

We thank the reviewers comments and blah, blah (INTRO)



Actually, in such a storage scheme biometric information would be stored in a decentralized public way. This is not recommendable and explicitly prohibited by privacy regulations.

A new 

Additions que hemos hecho:
· On-chain matching based on Euclidean and hamming distance.


Reviewer: 1

Recommendation: Reject

Comments:
The reviewer identifies several issues with this manuscript.

It is suggested to secure sensitive and private data stored in biometric template through blockchain technology (as stated in the abstract). Later in the introduction the authors mention that blockchain technology can be useful to secure biometric template and assure privacy in biometric systems. From given citations it becomes clear that the authors refer to biometric template protection. Template protection schemes are required to ensure irreversibility, unlinkability and renewability of biometric template and ideally preserve accuracy. In the concept introduced by the authors blockchain is utilized to protect the integrity of the biometric template. This should prevent from two attacks, "modify templates" in the database and "intercept channel" between database and matcher (6. and 7. in Fig. 1). Actually, this does not directly relate to template protection.

The authors give no explanation why a blockchain is required to achieve integrity protection. It is not clear to the reader why conventional cryptographic techniques which would be more efficient, e.g. signing of templates by a TTP, would not be enough in their scenario.

Three storage schemes are discussed by the authors. The first one suggests to directly store biometric templates in the blockchain which is identified as less efficient. Actually, in such a storage scheme biometric information would be stored in a decentralized public way. This is not recommendable and explicitly prohibited by privacy regulations. For instance, the EU suggests data  which is found to classify as personal data (like biometric data) be kept off-chain and merely link to the ledger through a hash-pointer.

The second and third scheme follow this principle and store hashes of biometric data in a blockchain. However, here is some major problem. As the authors correctly state, it is not possible to use secret keys in their architecture. Hence it is suggested to generate 256-bit hashes of the biometric template (with SHA3). It is crucial that the mere use of a hash function will not automatically transform personal data into anonymous data. For hashing to be non-invertible, the number of possible inputs must be sufficiently large and unpredictable to prevent the option of trying all  possible combinations. In case plain biometric information is hashed the number of possible inputs directly relate to the entropy of the biometric data which is obviously much lower than 256 bits considering the amount of used features in the presented case study. Moreover, biometric information (the hashes) do not fulfill the requirement of unlinkability which is essential to prevent from cross-matching attacks. 

Eventually, the deletion of biometric information becomes problematic in the proposed concept. As stated by the authors, template data remains in the blockchain even after deletion. This is another issue and clear limitation which contradicts to data privacy regulations.

Minor: the introductory section on blockchain would be rather redundant in this special issue.

Overall, this concept of combining biometrics with blockchain requires some major re-design to solve the mentioned issues. At the present state, it appears the proposed concept even reduces privacy protection and contradicts with existing data protection regulations, e.g. GDPR.

Additional Questions:
1. How relevant is this manuscript to the readers of this periodical? Please explain your rating in the Detailed Comments section.: Interesting - but not very relevant

1. Please summarize what you view as the key point(s) of the manuscript and the importance of the content to the readers of this periodical. If you don't have any comments, please type No Comments.: In this manuscript, the potential of combining biometric recognition with blockchain technology is investigated. After a introduction to both fields the authors discuss the possibility of storing (hashes of) biometric data in a blockchain. Subsequently, some trade-offs regarding biometric feature size and resulting costs of the proposed scheme are discussed.

2. Is the manuscript technically sound? Please explain your answer in the Detailed Comments section.: Partially

3. What do you see as this manuscript's contribution to the literature in this field?: The manuscript is basically an extension of a previously published conference paper. It makes the attempt of combining biometrics with blockchain technology.

4. What do you see as the strongest aspect of this manuscript?: The manuscript is well organized, clearly written and easy to follow.

5. What do you see as the weakest aspect of this manuscript?: Different essential aspects are not covered in this work which could have a severe impact on security/privacy.

1. Does the manuscript contain sufficient and appropriate references? Please elaborate in the Detailed Comments section.: References are sufficient and appropriate

2. Does the introduction state the objectives of the manuscript in terms that encourage the reader to read on? Please explain your answer in the Detailed Comments section.: Yes

3. How would you rate the organization of the manuscript? Please elaborate in the Detailed Comments section.: Satisfactory

4. Is the length of the manuscript appropriate for the topic? Please elaborate in the Detailed Comments section.: Satisfactory

5. Please rate the readability of this manuscript in the Detailed Comments section.: Easy to read

Please rate the manuscript. Explain your choice in the Detailed Comments section.: Poor


Reviewer: 2

Recommendation: Author Should Prepare A Major Revision For A Second Review

Comments:
This manuscript conducted a in-depth study on the application of blockchain technology in biometrics, with emphasis in biometric template storage and protection. Through experiments on Ethereum blockchain platform, this study has proved the feasibility of combining
both biometric and public blockchains in both economic and performance perspectives.

However, the new technical contribution in this journal manuscript is very limited, almost all of the technical research outcomes are from the conference paper. Authors need to develop some original research in this journal version.

Additional Questions:
1. How relevant is this manuscript to the readers of this periodical? Please explain your rating in the Detailed Comments section.: Relevant

1. Please summarize what you view as the key point(s) of the manuscript and the importance of the content to the readers of this periodical. If you don't have any comments, please type No Comments.: biometric template storage and protection

2. Is the manuscript technically sound? Please explain your answer in the Detailed Comments section.: Yes

3. What do you see as this manuscript's contribution to the literature in this field?: As claimed in the manuscript, this work is the first to conduct a in-depth study regarding the application of blockchain technology in biometrics, with emphasis in biometric template storage and protection. Through experiments on Ethereum blockchain platform, this study has proved the feasibility of combining
both biometric and public blockchains in both economic and performance perspectives.

4. What do you see as the strongest aspect of this manuscript?: The manuscript proposed to use Merkle trees as the intermediate data structure for the storage of biometrics.

Face and signature are used as the case study to evaluate the performance of operations and storage.

5. What do you see as the weakest aspect of this manuscript?: The new technical contribution in this journal manuscript is very limited, almost all of the technical research outcomes are from the conference paper. Authors need to develop some original research in this journal version.

1. Does the manuscript contain sufficient and appropriate references? Please elaborate in the Detailed Comments section.: References are sufficient and appropriate

2. Does the introduction state the objectives of the manuscript in terms that encourage the reader to read on? Please explain your answer in the Detailed Comments section.: Yes

3. How would you rate the organization of the manuscript? Please elaborate in the Detailed Comments section.: Satisfactory

4. Is the length of the manuscript appropriate for the topic? Please elaborate in the Detailed Comments section.: Satisfactory

5. Please rate the readability of this manuscript in the Detailed Comments section.: Easy to read

Please rate the manuscript. Explain your choice in the Detailed Comments section.: Good


Reviewer: 3

Recommendation: Reject

Comments:
The paper describes the use case involving biometrics and blockchain. The list of pros and cons is quite nice and comprehensive. I had expected to see some tech contributions of combining the two areas but the authors are basically considering the biometric templates as a database and discuss ways of dealing with storing a database within a blockchain framework. The same discussion and observations in the paper hold for any database. There is no novelty here and no discussion on how to create a synergy between blockchain and biometrics.
I was expecting to see unique features enabled by the integration of biometrics with the blockchain tech (e.g., SMC, private matching, etc.), but the paper contains only a discussion of known ways for dealing with storing a large database within the blockchain framework.

Additional Questions:
1. How relevant is this manuscript to the readers of this periodical? Please explain your rating in the Detailed Comments section.: Relevant

1. Please summarize what you view as the key point(s) of the manuscript and the importance of the content to the readers of this periodical. If you don't have any comments, please type No Comments.: The paper discusses the pros and cons of integrating blockchain with biometrics.

2. Is the manuscript technically sound? Please explain your answer in the Detailed Comments section.: Yes

3. What do you see as this manuscript's contribution to the literature in this field?: The paper discusses the pros and cons of integrating blockchain with biometrics.

4. What do you see as the strongest aspect of this manuscript?:

5. What do you see as the weakest aspect of this manuscript?:

1. Does the manuscript contain sufficient and appropriate references? Please elaborate in the Detailed Comments section.: Important references are missing; more references are needed

2. Does the introduction state the objectives of the manuscript in terms that encourage the reader to read on? Please explain your answer in the Detailed Comments section.: Could be improved

3. How would you rate the organization of the manuscript? Please elaborate in the Detailed Comments section.: Could be improved

4. Is the length of the manuscript appropriate for the topic? Please elaborate in the Detailed Comments section.: Could be improved

5. Please rate the readability of this manuscript in the Detailed Comments section.: Easy to read

Please rate the manuscript. Explain your choice in the Detailed Comments section.: Poor


